Operationalizing Counterfactual Metrics: Incentives, Ranking, and Information Asymmetry

From the social sciences to machine learning, it has been well documented that metrics to be optimized are not always aligned with social welfare. In healthcare, Dranove et al. (2003) showed that publishing surgery mortality metrics actually harmed the welfare of sicker patients by increasing provider selection behavior. We analyze the incentive misalignments that arise from such average treated outcome metrics, and show that the incentives driving treatment decisions would align with maximizing total patient welfare if the metrics (i) accounted for counterfactual untreated outcomes and (ii) considered total welfare instead of averaging over treated patients. Operationalizing this, we show how counterfactual metrics can be modified to behave reasonably in patient-facing ranking systems. Extending to realistic settings when providers observe more about patients than the regulatory agencies do, we bound the decay in performance by the degree of information asymmetry between principal and agent. In doing so, our model connects principal-agent information asymmetry with unobserved heterogeneity in causal inference.

==> sections/abstract.tex <==
%%%% Original introduction focused on accountability %%%%

Public accountability metrics and rankings for healthcare providers have become increasingly influential in the US in the last few decades. While deployed with goals of improving patient safety, the actual effects of these metrics on patient welfare have been mixed, with \citet{dranove2003more} showing that metrics actually harmed the welfare of sicker patients by increasing provider selection behavior.
Using a principal agent model, we directly study the incentive misalignments that arise for different accountability metrics, and show that the incentives driving treatment decisions would align with maximizing total patient welfare if the metrics \textit{(i)} accounted for counterfactual untreated outcomes and \textit{(ii)} considered total welfare instead of average welfare among treated patients.
Operationalizing this, we show how counterfactual measures can be modified to satisfy desirable properties when used as ranking metrics. Extending to realistic settings when the providers observe more about patients than the regulatory agencies do, we bound the decay in performance by the degree of information asymmetry between the principal and the agent. In doing so, our model directly connects information asymmetry in a principal agent game with unobserved heterogeneity in causal inference. 

==> sections/intro.tex <==
%%%% Original introduction focused on accountability %%%%

\section{Introduction}

%%%% Healthcare report cards motivation %%%%

The publication of accountability and quality metrics for healthcare providers has been both prevalent and contentious in the US since the 1990s.
As an early pioneering example, the New York Health Department published mortality rates for a cardiac procedure per physician and hospital, and \citet{dranove2003more} showed that the publication of these metrics by the health departments actually harmed the welfare of sick patients by increasing selection behavior from providers. Specifically, providers had an incentive to selectively treat healthier patients with a lower probability of mortality instead of sicker patients that would have benefited more from treatment.

Today's healthcare accountability metrics continue to rely heavily on \textit{average treated outcome} measures. Medicare compensation for doctors depends on estimates of the average outcomes of the treated patients for different procedures \cite{mips}, in a similar fashion to the New York Health Department's initially published mortality rates. Similarly, \citet{glance2021association} showed that these scores do not always correlate with better health outcomes for patients. 

The uncertainty surrounding the efficacy of these accountability metrics has not prevented their continued growth and usage. In the last decade, the Centers for Medicare and Medicaid Services (CMS) has spent \$1.3 billion to develop quality measures for physicians and hospitals
% , and physicians spent an average of 15 hours per week reporting quality scores in 2014 
\citep{wadhera2020quality,casalino2016us}. In addition to determining Medicare compensation for doctors \cite{mips}, CMS metrics are applied in many public facing ranking systems by private and government organizations such as the US News and World Report, the LeapFrog Hospital Safety Score, and Cal Hospital Compare \citep{nyt,calhospitalcompare}. While deployed with ambitious goals of improving patient safety \cite{donaldson2000err}, many medical studies have questioned the relationship between these ranking measures and patient outcomes~\citep[see,e.g.,][]{gonzalez2014hospital,ryan2009relationship,hwang2014hospital, jha2008does,smith2017dissecting}.

%%%% Incentive alignment by incorporating counterfactual estimates into the metrics %%%%

In this work, we directly study the incentive misalignment when \textit{average treated outcome} measures are used as quality and accountability metrics, and consider how total welfare might improve if \textit{causal effects} were measured and reported instead. Our work formally analyzes and operationalizes the insight that if accountability metrics were to include causal estimates of treatment effects, then the incentives driving the provider's treatment decisions can be aligned with maximizing total welfare. 
 
%%%% Broader applications to ranking problems with treatment selection %%%%

% More generally, we analyze the welfare effects of accountability metrics
More generally, our analysis applies to any environment where accountability metrics are learned from data over which the measured agent can exercise some control. We refer to healthcare metrics as a running example where these effects are well documented; however, our model generally applies to any multi-agent environment with treatment selection. Other domains subject to this phenomenon include education, where ranking and algorithmic accountability measures are applied to institutions that can select whom to admit; and online ranking platforms for businesses that may exercise some selection power over their customers, such as restaurants, hotels, and independent contractors. Such ranking platforms have significant sway in the operations of these organizations \cite{mau2019metric,ursu2018power}, which means that the ranking metrics themselves have critical downstream impacts on user welfare.

%%%% Preview of model and results %%%%%
To study the welfare effects that arise from this dynamic interaction between accountability metrics and providers, we employ a \textit{principal-agent model} where the \textit{principal} chooses a quality measure as a reward function, and the \textit{agent} responds by optimizing this reward function to the best of their private abilities and information. To analyze the welfare effects of reward policy choices, we apply a causal framework similar to that of policy learning and policy evaluation, where the goal is to allocate treatments that maximize the total positive effects over a population relative to treating no one \cite{manski2008identification}. 

\textbf{Contributions.} We show that \textit{average treated outcome} measures incur unbounded regret by this definition of welfare, and show that regret can be reduced by \textit{(i)} accounting for counterfactual untreated outcomes and \textit{(ii)} considering total welfare instead of average welfare among treated patients. Applying these two simple insights yields an optimal functional form for a quality measure that achieves zero regret as long as the principal can learn the mean conditional untreated potential outcomes. We refer to this as rewarding the \textit{total treatment effect}. 

Connecting this theoretical result to practice, we discuss two issues that arise when operationalizing the total treatment effect measure in realistic applications. First, we study the complications that arise when the total treatment effect is used to \textit{rank} different agents that might have different treatment population sizes and distributions, such as hospitals that serve more under-resourced populations. We show that the total treatment effect measure can be adjusted to yield rankings that account for these differences. Second, we consider practical issues of \textit{information asymmetry}, where the agent might observe more features about each patient than the principal. We bound the decay in performance as the severity of information asymmetry increases. In doing so, our model connects information asymmetry in this principal-agent model to unobserved heterogeneity in causal inference, opening the door to future technical work that could more deeply leverage this connection. 

Finally, we empirically compute regrets of different quality measures over two real  clinical datasets. In addition to confirming that the average treated outcome indeed incurs high regret, we show that the principal can do reasonably well knowing only a subset of the total set of features. 

